Spectral Methods for Correlated Topic Models

In this paper, we propose guaranteed spectral methods for learning a broad range of topic models, which generalize the popular Latent Dirichlet Allocation (LDA). We overcome the limitation of LDA to incorporate arbitrary topic correlations, by assuming that the hidden topic proportions are drawn from a flexible class of Normalized Infinitely Divisible (NID) distributions. NID distributions are generated through the process of normalizing a family of independent Infinitely Divisible (ID) random variables. The Dirichlet distribution is a special case obtained by normalizing a set of Gamma random variables. We prove that this flexible topic model class can be learned via spectral methods using only moments up to the third order, with (low order) polynomial sample and computational complexity. The proof is based on a key new technique derived here that allows us to diagonalize the moments of the NID distribution through an efficient procedure that requires evaluating only univariate integrals, despite the fact that we are handling high dimensional multivariate moments. In order to assess the performance of our proposed Latent NID topic model, we use two real datasets of articles collected from New York Times and Pubmed. Our experiments yield improved perplexity on both datasets compared with the baseline.

==> Extensions.tex <==
\section{Outline}

 \input{NID.tex}

\subsection{Dirichlet Process}
According to \cite{ishwaran2002exact}, the Dirichlet process is an infinite limit of the Dirichlet distribution when represented in the mixture form representation of
\begin{equation}
	\mathcal{P}_k(\cdot) = \sum \limits_{i \in k} h_i \delta_{z_i}(\cdot)
\end{equation}
where the weights $h_i$ are drawn from the $\text{Dir} (\mathbf{\alphabf})$ distribution and $z_i$'s are points drawn iid from an underlying distribution $\mathcal{H}$. $k$ represents the number of components or the dimensionality of the Dirichlet distribution and $\mathbf{\alphabf} = (\alpha_0/k, \dots, \alpha_0/k)$. It is proven that $\lim_{k \rightarrow \infty} \mathcal{P}_k$ tends to the Dirichlet process $\text{DP}(\mathbf{\alphabf} \mathcal{H})$ in distribution that is represented as
\begin{equation}
\label{eq:DP}
	\mathcal{P} (\cdot) = \sum \limits_{i = 1}^{\infty} h_i \delta_{z_i}(\cdot)
\end{equation}
Campbell et. al. \cite{campbell2016truncated} give a detailed description of the truncation analysis of random measures.

\begin{lemma} ({\textbf{Separability under the Dirichlet Process}})
\label{lem:DP}
Let $\Psi(s,\bm u)$ indicate the modified second characteristic function of the Dirichlet process in Equation \eqref{eq:DP}. Then since the DP is an infinite limit of the Dirichlet distribution we have
\begin{align}
\label{eq:charac}
	\Psi(s,\uv) & = \log \big[ \mathcal{L}_t \{ t^{\alpha_0-1} \psi_h(t \uv) ; s\} \big] = \log  \bigg[ \mathcal{L}_t \big\{ t^{\alpha_0-1} \mathbb{E}[ e^{i\langle{t \uv},{ \hv}\rangle}] ; s \big\} \bigg] \nonumber \\
	%
	 &= \sum \limits_{j = 1}^\infty \log \bigg[ \int \limits_0^\infty \big(h_j^{-1} e^{(i u_j-s) h_j} \big) \mathrm d h_j \bigg] - \log [B],
\end{align}
where $\uv \in \mathbb{R}^k$ and $B$ is the normalization factor of the distribution.
% and $0 \leq m \leq N-k-1$ with $N$ indicating the total number of samples drawn from Gibbs.
%As a consequence, weights $v_1$ and $v_2$ in Theorem \ref{thm:mainResult} are of the following form
%\begin{align}
% v_1  = \frac{- \mathcal{L}_t \big\{ t^{\alpha_0} \big\} \cdot \mathcal{L}_t \big\{ t^{\alpha_0+1} \big\}}{\mathcal{L}_t \{ t^{\alpha_0-1} \} \cdot \mathcal{L}_t \big\{ t^{\alpha_0+2} \big\}} \qquad \qquad
% v_2  = \frac{2 \big(\mathcal{L}_t \{t^{\alpha_0} \}\big)^3}{\big(\mathcal{L}_t \{t^{\alpha_0-1} \}\big)^2 \cdot \mathcal{L}_t \big\{ t^{\alpha_0+2} \big\}}
%\end{align}
\end{lemma}
 
 \subsection{Projecting Independent Draws onto the Simplex}
According to the stick-breaking construction of the Dirichlet distribution, one can draw samples independently from the Gamma distribution and then normalize the draws with their sum. In this section we will see how the Gamma distribution draws lead to the results of the previous section and how we can use other distributions to generalize our results.

Consider that variables $w_i$ for $i \in [k]$ are drawn independently from the $\Gamma(\alpha, \beta)$ distribution shown below
\begin{equation}
\label{eq:pdfGamma}
	\Pr(w_i) = \frac{\beta^\alpha}{\Gamma(\alpha)} w_i^{\alpha-1} e^{- \beta w_i} \qquad \qquad \alpha>0, \; \; \beta>0
\end{equation}
Then variables $h_i = \frac{w_i}{Z}$, where $Z = \sum_{i \in [k]} w_i$ are Dirichlet distributed on the simplex.

\subsection{Gibbs Process}
The Gibbs process is a class of exchangeable probability partition that includes processes such as the Dirichlet process and the Pitman-Yor process. These probability partitions can be uniquely represented by their Exchangeable Partition Probability Function (EPPF) According to \cite{gnedin2006exchangeable} the EPPF of Gibbs processes have a special product form. These class of distributions, impose exchangeable partitions on the natural numbers and can be used in non-parametric Bayesian analysis as the prior for mixture modeling. These processes are of discrete nature and we would like to investigate the possibility of representing the Gibbs process as a griddified version of the Dirichlet distribution, and generalize its results to the Gibbs processes.  

\paragraph{Note:} Mixture inconsistency of the Dirichlet process \cite{miller2013simple}.

==> graphical_model.tex <==
\tikzset{
	regS/.style = {  },
	aliasS/.style = {double = black!0, double distance=1.2pt},
%	aliasS/.style = {},
%	minustS/.style = {double = black!30, double distance=1pt}
	%double/.style = {double = black!40, double distance=1.2pt}
}
\begin{tikzpicture}
[ ->,>=stealth',shorten >=1pt,auto,node distance=1.2cm,
  %thick
  ,main node/.style={circle,fill=black!20,draw,
  font=\sffamily\small\bfseries
  },
   minimum size=.6cm
   ,inner sep=2pt
   ]
  \node[main node] (p)  {$\hv$};
	\node[main node] (t1) [below left = .4cm and 1.5cm  of p] {$y_1$};
	\node[main node] (t2) [below left = .4cm and .25cm  of p] {$y_2$};
	\node (tdots) [below right = .4cm and .25cm  of p] {$\dots$};
	\node[main node] (tn) [below right = .4cm and 1.5cm  of p] {$y_l$};
	
	\node[main node] (x1) [below = .4cm of t1] {$\xv_1$};
	\node[main node] (x2) [below = .4cm of t2] {$\xv_2$};
	\node (xdots) [below = .4cm of tdots] {$\dots$};
	\node[main node] (xn) [below = .4cm of tn] {$\xv_l$};
	
	\path[] 
		(p) edge node {} (t1)
		(p) edge node {} (t2)
		(p) edge node {} (tn)
		;
	
	\path[] 
		(t1) edge node {} (x1)
		(t2) edge node {} (x2)
		(tn) edge node {} (xn)
		;

	\node (textP) [right = .25cm of p] {$\sim \Pr(\hv)$};
	\node (textTn) [right = .25cm of tn] {$y_i \sim \text{multinomial}(\hv)$};
	\node (textTn) [right = .25cm of xn] {$\xv_i \sim \text{multinomial}( A_{y_i})$};
	
	
	\node (textPL) [left = .25cm of p] {distribution over topics}; 
	\node (textTn) [left = .25cm of t1] {topics};
	\node (textTn) [left = .25cm of x1] {words};
	
	%\node[main node, double = black!40, double distance=1.2pt] (3) [below of = 2] {3};
  %\node[main node] (4) [below of=1, double = black!40, double distance=1.2pt] {4};
  %

  %\path[every node/.style={font=\sffamily\small}]
    %(1) %edge node [left] {0.6} (4)
        %edge [bend left] node[above] {\tiny $.6$} (2)
				%edge [bend left] node[left] {\tiny $.1$} (4)
        %%edge [loop left] (1)
    %(2) %edge node [right] {0.4} (1)
        %%edge node {0.3} (4)
        %%edge [loop right] node[right] {} (2)
        %edge [bend left] node[right] {\tiny $.5$} (3)
				%edge [bend left] node[above] {\tiny $.25$} (1)
    %(3) %edge node [right] {0.8} (2)
    		%%edge [loop right] node[below] {} (3)
        %edge [bend left] node[below] {\tiny $.7$} (4)
				%edge [bend left] node[right] {\tiny $.2$} (2)
    %(4) %edge node [left] {0.2} (3)
        %%edge [loop left] node[left] {} (4)
        %edge [bend left] node[left] {\tiny $.8$} (1)
				%edge [bend left] node[below] {\tiny $.1$} (3);

%[scale = 1.1,
%every node/.style = {draw, shape = circle, minimum size = 5.mm,inner sep = 0mm, fill = black!0}
%]
%\node [regS] (s1) at (-1,0) {$1$};
%\node [aliasS] (s2) at (0,1) {$2$};
%\node [regS] (s3) at (1,0) {$3$};
%\node [aliasS] (s4) at (0,-1) {$4$};
%%\draw  [dashed] (m1) -- (p1) node [left=7pt, midway, draw=none, fill = none] {$(S)$};
%%\draw  [dashed](p2) -- (m2) node [above right=18pt,draw=none, fill = none] {$(\tilde S)$};
\end{tikzpicture}


==> inference.tex <==
\section*{Inference Using MCMC sampling}
The problem of inference reduces to the problem of inferring the hidden topic assignments per document, $\hv$, and the hidden topic-word assignments per each word in the document, $\zetabf$. In other words we need to compute the following posterior distribution given the word counts vector $\mathbf{w^{(d)}}$ for document $d \in [D]$,
\begin{align}
	\Pr(\hv, \zetabf) & = \frac{\Pr(\hv,\zetabf,\mathbf{w} \vert \alphabf, \Am)}{\Pr(\mathbf{w} \vert \alphabf, \Am)} \nonumber \\
	& = \frac{\Pr(\hv,\zetabf,\mathbf{w} \vert \alphabf, \Am)}{\int \sum_{\zetabf} \Pr(\hv,\zetabf,\mathbf{w} \vert \alphabf, \Am) \mathrm{d} \hv}.
\end{align}
The denominator is in general intractable under different prior distributions and needs to be approximated using different techniques such as variational inference \cite{blei2003latent,blei2006correlated}, or MCMC sampling \cite{griffiths2004finding, mimno2008gibbs, chen2013scalable}.

As it is known, NID distributions do not have closed form representations in general. Variational inference methods, on the other hand, need to have access to the distribution's closed form. Therefore, they do not seem to be a good candidate for our topic model under NID priors. In stead, we will use an MCMC Metropolis-Hastings sampler for inferring the hidden variables given each document $\mathbf{w}$ and the estimated parameters $\alphabf$ and $\Am$.

%In order to perform MCMC Gibbs sampling, we need to compute the following full conditionals,
%\begin{align}
%	& \Pr(z_i = j \vert \mathbf{z}_{-i}, \hv, \mathbf{w}, \alphabf, \Am)
%	\label{eq:zInfer} \\
%	& \Pr(h_j = t \vert \mathbf{z}, \hv_{-j}, \mathbf{w}, \alphabf, \Am)
%	\label{eq:hInfer}
%\end{align}

Let $\mathbf{w}^{(d)} \in \mathbb{R}^V$ indicate the vector of word counts for document $d$ of length $N$ in the corpus and let $\hv^{(d)} \in \mathbb{R}^k$ denote the hidden topic proportions of document $d$. The posterior distribution is represented below
%These conditionals can be computed from the joint posterior $\Pr(\mathbf{z},\hv \vert \mathbf{w}, \alphabf, \Am)$ by collecting the terms that depend on $z_i$ and $h_j$ ignoring the constant terms and guessing what the underlying distribution of each conditional is. We have
\begin{align}
	& \Pr(\zetabf, \hv^{(d)} \vert \mathbf{w}^{(d)}, \alphabf, \Am) = \frac{\Pr(\zetabf, \hv^{(d)}, \mathbf{w}^{(d)} \vert \alphabf, \Am)}{\Pr(\mathbf{w}^{(d)}, \vert \alphabf, \Am)} \nonumber \\
	& \propto \Pr(\zetabf, \hv^{(d)}, \mathbf{w}^{(d)} \vert \alphabf, \Am) \nonumber \\
	& = \Pr(\hv^{(d)} \vert \alphabf) \prod_{n \in N} \Pr(\zeta_n^{(d)} \vert \hv^{(d)}) \Pr(w_n^{(d)} \vert \zeta_n^{(d)}, \Am) \nonumber \\
	& = \int \limits_0^\infty \prod_{i \in [k-1]} f_i(h_i m) f_k(m - \sum_{i \in [k-1]} h_i m) m^{k-1} \mathrm{d} m \nonumber \nonumber \\ 
	& \times \prod_{i \in [k]} h_i^{n_{d,i}} \prod_{i \in [k]} \prod_{j \in V} (A_{i,j})^{n_{i,j}},
	\label{eq:posterior}
\end{align}
where $f_i(\cdot)$ indicates the distribution of the original ID variable, $n_{d,i}$ denotes the number of words assigned to topic $i$ in document $d$ and $n_{i,j}$ indicates the number of times word $j$ is assigned to topic $i$. Normally in topic modeling settings $\hv$ would integrate out making Gibbs sampling possible. Here, however, the full conditional will not yield a known distribution to draw samples from. Therefore, one needs to perform Metropolis-Hastings MCMC to be able to generate draws from the posterior \eqref{eq:posterior} and perform inference. 

It should be noted that for topic models such as Latent Dirichlet Allocation \cite{griffiths2004finding} and Correlated Topic Models \cite{mimno2008gibbs} (that assumes that the topics are drawn from the Logistic-Normal) distribution, the Dirichlet distributed parameters can be integrated out and we only need to infer $\zetabf$. This is not the case in our topic modeling scenario, however. The posterior inference algorithm is given in Algorithm \ref{alg:inference}. The jumping distribution is chosen to be that of the Dirichlet distribution to ensure that the topics lie on a simplex and the hidden topics are drawn from a multinomial distribution whose parameters have been estimated in the learning stage.

\input{inferenceAlg.tex}

==> inferenceAlg.tex <==
\begin{algorithm}
\caption{Posterior inference using MCMC Metropolis-Hastings algorithm}
\label{alg:inference}
\begin{algorithmic}[1]
%Let $\yv = (y_1,y_2, \dots, \y_k)$
\Require Word count vector $\mathbf{w}^{(d)}$, $\alphabf$ and $\Am$
\Ensure $T$ samples from latent topic assignments $\zetabf$, latent topic proportions $\hv^{(d)}$ and counts $n_{d,i}$ and $n_{i,j}$ for $i \in [k]$ and $j \in V$
\State Randomly initialize  $\zetabf$ and $\hv^{(d)}$ and compute $n_{d,i}$ and $n_i,j$
\For{t = 1:T}
	\State //Step 1: Generate a candidate sample from any jumping distribution $J_t(\hv^*,\zeta_n^* \vert \hv^{(t-1)},\zeta_n^{(t-1)})$
	\State $\hv^* \gets$ Draw a sample from Dir$(\alphabf + n_{d,\cdot})$
	\For{n = 1:N}
		\State $w_n \gets \mathbf{w}[n]$
		\State $\zeta_n^* \gets$ Draw a sample from Mult$(1,A_{\hv^*})$
	\EndFor
	\State Update counts $n_{d,i}$ and $n_{i,j}$
	\State //Step 2: Compute acceptance ratio $r$
	\State $r = \frac{\Pr(\hv^*,\zeta_n^* \vert \mathbf{w}^{(d)}, \alphabf,\Am) / J_t(\hv^*,\zeta_n^* \vert \hv^{(t-1)},\zeta_n^{(t-1)})}{\Pr(\hv^{(t-1)},\zeta_n^{(t-1)} \vert \mathbf{w}^{(d)}, \alphabf,\Am) / J_t(\hv^{(t-1)},\zeta_n^{(t-1)} \vert \hv^*,\zeta_n^*)}$
	\State //Step 3: Accept or reject the drawn sample
	\State $u \gets$ Draw a sample from Uniform$(0,1)$
	\If {$u \leq r$}
		\State $\hv^{(t)} \gets \hv^*$
		\State $\zeta_n^{(t)} \gets \zeta_n^*$
	\Else 
		\State $\hv^{(t)} \gets \hv^{(t-1)}$
		\State $\zeta_n^{(t)} \gets \zeta_n^{(t-1)}$
	\EndIf
\EndFor
\end{algorithmic}
\end{algorithm}

==> notation.tex <==
\paragraph{Notation: } Let $[k]:=\{1, \ldots, k\}$.  We use the convention of~\cite{ragnarsson2012block} to obtain transpositions of a tensor $T$
\beq T^{\inner{p}}(i_{p_1}, i_{p_2}, \ldots) = T(i_1, i_2, \ldots), \label{eqn:transpose}\eeq where $p$ is a permutation. For example, for a second order tensor (i.e a matrix) $M$ and $p=\{2,1\}$, we have $M^{\inner{p}}= M^\top$. For a  third order tensor $T$, if $p=\{2,3,1\}$, we have the  $T^{\inner{p}}(i_2, i_3, i_1) = T(i_1, i_2, i_3)$.
We will also use the symmetrized form of a tensor \beq\symm(T):=\sum_p T^{\inner{p}},\label{eqn:symm}\eeq where the sum is over all the permutations. Note that $\symm(T)$ is a supersymmetric tensor, e.g. for a matrix $M$, $\symm(M)= M + M^\top$.



==> response.tex <==
\subsection*{Response to NIPS reviewers:}
The NIPS reviews have been very helpful and accurate. In this revision we have addressed the minor and major concerns. The major concern was the lack of experimental results. We have added experimental results on two different text corpora, namely New York Times and Pubmed. We use the well-known perplexity measure to assess the goodness of fit and also output the topics  returned  by the algorithm.

Below we provide detailed response to the questions raised by NIPS reviewers. We would like to also note that the comments have been applied to the current version submitted to AISTATS 2017. Detailed response to the reviewer's comments are given below:

\paragraph{Experiments: } The focus of the original submitted paper was theoretical. We are adding experimental results to this version of the paper since most of the reviewers where curious to see the performance of our proposed method on real data. We have added a new section and experiments on two real-world datasets to the paper to address this issue. 

\paragraph{Modeling both positive/negative correlations:} In figure 3, we plot proportion of positively correlated elements, i.e. out of all n choose 2 correlations among n variables, we plot proportion of how many elements are positive. As u can see for certain ID distributions such as inverse Gaussian, there can be both positive and negative correlations. On the other hand, Dirichlet only has negative correlations which is limiting.

\paragraph{Correlated topic model vs. NID:} There is currently no method for learning Correlated Topic Models with guarantees. Spectral methods are efficient and provide guarantees, yet they cannot be easily adapted to Correlated Topic Models. On the other hand, NID models have best of both worlds: flexibility in modeling arbitrary correlations and also efficient learning with spectral methods. Furthermore, as discussed by \cite{passos2011correlations}, Correlated Topic Models give rise to spurious correlations that are undesirable.

\paragraph{Estimating the Levy measure:} This is discussed in detail in the Experiments section. One can tune for hyperparameters $v,v_1,v_2$ during the tensor decomposition algorithm. We will then fit the levy measure to the recovered $v, v_1$ and $v_2$ such that the penalized norm projection of the L\'{e}vy measure is minimized while maintaining a good likelihood. 

\paragraph{Novelty:} It is highly non trivial to show that the moments of all NID distributions can be diagonalized. Earlier spectral work directly works only on Dirichlet moments. We now provide an automated method to find the appropriate moment forms which are diagonalized for a broad family.

We provide detailed comments to each reviewer's comments below:

\paragraph{Reviewer 2: }
In order to ensure learnability we need the columns of matrix $A \in R^{d \times k}$ to be linearly independent and the parameters $\alpha_i > 0$. This is a very good point and we have added this assumption.

The proof for the correspondence of $\alpha_i$'s to the CP weights follows directly, but it has been added to the appendix for more clarity.

\paragraph{Reviewer 3: }
The reviewer makes an interesting point that the dependence on the underlying levy measure is through $v, v_1$ and $v_2.$ If we choose a wrong $v,v_1,v_2,$ in general we would not be getting a low rank representation and hence will not be able to learn the correct model. It is an interesting open question, if there can be another configuration of $v,v_1,v_2$ that makes the resulting tensor low rank. It does not appear to be the case. We have added comments about this in the hyperparameter tuning section in the experimental results.

%\paragraph{Reviewer 4: }	We will add the work on NMF to revised version, which is complementary to this framework. NMF requires anchor word/separability assumption while tensor based methods do not require that. We will compare the two in future.

\paragraph{Reviewer 5: }
Many machine learning researchers may not be aware of NID distributions, and hence we provided a background section .We have added the mentioned reference.

\paragraph{Reviewer 6: }
Our main contribution is the spectral method and that is novel and nontrivial as discussed in the beginning. We have added more discussion about the NID distributions itself and compared them to other correlated topic models in revised version.




